DyNCA: Real-time Dynamic Texture Synthesis Using Neural Cellular Automata

Current Dynamic Texture Synthesis (DyTS) models can synthesize realistic videos. However, they require a slow iterative optimization process to synthesize a single fixed-size short video, and they do not offer any post-training control over the synthesis process. We propose Dynamic Neural Cellular Automata (DyNCA), a framework for real-time and controllable dynamic texture synthesis. Our method is built upon the recently introduced NCA models and can synthesize infinitely long and arbitrary-sized realistic video textures in real time. We quantitatively and qualitatively evaluate our model and show that our synthesized videos appear more realistic than the existing results. We improve the SOTA DyTS performance by $2\sim 4$ orders of magnitude. Moreover, our model offers several real-time video controls including motion speed, motion direction, and an editing brush tool. We exhibit our trained models in an online interactive demo that runs on local hardware and is accessible on personal computers and smartphones.

==> figures/Experiments/MotionVidDST.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \newcommand{\imgteaser}[1]{\includegraphics[height=75pt]{figures/teaser/#1}}
% \newcommand{\imgmvid}[1]{\includegraphics[height=75pt]{figures/Experiments/MotionVid/#1}}
% \newcommand{\imgteaserS}[1]{\includegraphics[height=55pt]{figures/teaser/#1}}
% \newcommand{\imgteaserM}[1]{\includegraphics[height=68pt]{figures/teaser/#1}}

\newcolumntype{G}{>{\centering\arraybackslash} m{75pt} }  %# New column type
\newcolumntype{F}{>{\centering\arraybackslash} m{80pt} }  %# New column type

% \newcommand{\arrow}{\textcolor{black}{\Longrightarrow}}%
% \newcommand{\ofarrow}{\hspace*{-8pt}$ \overset{OF}{\arrow}$}



\begin{table*}[]
\begin{tabular}{m{3pt}F|Gm{0pt}G|||Gm{0pt}G}
    
    
    \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Target Appearance}}} & \multicolumn{3}{c|||}{\hspace{-8pt}\textbf{Target Dynamic}} & \multicolumn{3}{c}{\hspace{-4pt}\textbf{Synthesized result}} \\
    
    \vspace{18pt}
    
    
    &                                    & Video     &        & Optic Flow     & Video      &        & Optic Flow     \\
    \midrule

(a) & \imgmvid{flames-cartoon_fire_1.png}                                & \imgmvid{flames-cartoon_fire_1_target.png}      &     \ofarrow   & \imgmvid{flames-cartoon_fire_1_targetflow.png}            & \imgmvid{flames-cartoon_fire_1_gen.png}        & \ofarrow     & \imgmvid{flames-cartoon_fire_1_genflow.png}            \\

(b) & \imgmvid{sea_2-cartoon_water_3.png}                                & \imgmvid{sea_2-cartoon_water_3_target.png}      &     \ofarrow   & \imgmvid{sea_2-cartoon_water_3_targetflow.png}            & \imgmvid{sea_2-cartoon_water_3_gen.png}        & \ofarrow     & \imgmvid{sea_2-cartoon_water_3_genflow.png}            \\

% (c) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     \ofarrow   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & \ofarrow     & \imgteaser{1.jpeg}            \\

% (c) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     \ofarrow   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & \ofarrow     & \imgteaser{1.jpeg}            \\

% (d) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     ==   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & ==     & \imgteaser{1.jpeg}            \\    
\end{tabular}
\caption{Results of dynamic style transfer with DyNCA. From the optic flow visualization, we can see that DyNCA does not simply try to copy the motion from the video but grab the style of the given motion information and make it naturally adapt to the target appearance.}
\label{tab:dynamic-style-transfer}
\end{table*}




==> figures/teaser.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\newcommand{\imgteaser}[1]{\includegraphics[height=75pt]{figures/teaser/#1}}
\newcommand{\imgteaserS}[1]{\includegraphics[height=55pt]{figures/teaser/#1}}
\newcommand{\imgteaserM}[1]{\includegraphics[height=68pt]{figures/teaser/#1}}




\begin{table*}[]
\begin{tabular}{m{3pt}F|Gm{0pt}G|||Gm{0pt}G}
    
    
    \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Target Appearance}}} & \multicolumn{3}{c|||}{\hspace{-8pt}\textbf{Target Dynamic}} & \multicolumn{3}{c}{\hspace{-4pt}\textbf{Synthesized result}} \\
    
    \vspace{18pt}
    
    
    &                                    & Video     &        & Optic Flow     & Video      &        & Optic Flow     \\
    \midrule
    
(a) & \imgteaser{bubble_app.jpg}                                & \imgteaserS{none.png}      &       & \imgteaserM{target_flow.png}            & \imgteaser{bubble_synth.png}        & \ofarrow     & \imgteaser{bubble_synth_flow.png}            \\


(b) & \imgteaser{flag_app.png}                                & \imgteaser{flag_target.png}      &     \ofarrow   & \imgteaser{flag_target_flow.png}            & \imgteaser{flag_synth.png}        & \ofarrow     & \imgteaser{flag_synth_flow.png}            \\

% (c) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     \ofarrow   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & \ofarrow     & \imgteaser{1.jpeg}            \\

% (c) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     \ofarrow   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & \ofarrow     & \imgteaser{1.jpeg}            \\

% (d) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     ==   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & ==     & \imgteaser{1.jpeg}            \\    
\end{tabular}
\caption{1. Difference between optic flow (comparable) 2. Dynamic style transfer on second row}
\end{table*}




==> sections/methods/FinalObj.tex <==
\subsection{Final Objectives}
\label{sec:finalobj}

$\mathcal{L}=\mathcal{L}_{appr}+\alpha \mathcal{L}_{motion}+\beta \mathcal{L}_{overflow}$

Different $\mathcal{L}_{motion}$ for different objectives.

==> tables/performance_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{table}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
% \begin{tabular}[c]{@{}c@{}}\textbf{Sketch Synthesis} \\ \textbf{Algorithms}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}{Method}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}{Training time/frame}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}{Synthesizing time/frame}\end{tabular} 
&\begin{tabular}[c]{@{}c@{}}{C}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{D}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{E}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{F}\end{tabular} \\
\begin{tabular}[c]{@{}c@{}}{\textbf{G}}\end{tabular} & \\

\midrule 

Tesfaldet et al. \cite{two_stream} &\xmark & \cmark \\

Xie et al. \cite{xie2017generativeconvnet} &\xmark & \xmark \\

\midrule
\textbf{Ours} & \cmark & \cmark \\
\bottomrule
\end{tabular}
}
% \vspace{-5pt}
\caption{Comparison of the speed of training a dynamic texture synthesis model and synthesizing videos with it.}
\label{tab:sketch_synth_comparison}
\end{table}

% Comparison of GAN-based image editing algorithms by their characteristics. \fbox{\textbf{A}} Works on any Dataset, \fbox{\textbf{B}} No test-time optimization, \fbox{\textbf{C}} Works on any GAN architecture, \fbox{\textbf{D}} Can perform the edit using a single image, \fbox{\textbf{E}} Allows global semantic editing, \fbox{\textbf{F}} Allows localized semantic editing, \fbox{\textbf{G}} Allows editing any object in the image


